Digital Contact Tracing: Technologies, Shortcomings, and the Path Forward

Since the start of the COVID-19 pandemic, technology enthusiasts have pushed for digital contact tracing as a critical tool for breaking the COVID-19 transmission chains. Motivated by this push, many countries and companies have created apps that enable digital contact tracing with the goal to identify the chain of transmission from an infected individual to others and enable early quarantine. Digital contact tracing applications like AarogyaSetu in India, TraceTogether in Singapore, SwissCovid in Switzerland, and others have been downloaded hundreds of millions of times. Yet, this technology hasn't seen the impact that we envisioned at the start of the pandemic. Some countries have rolled back their apps, while others have seen low adoption. Therefore, it is prudent to ask what the technology landscape of contact-tracing looks like and what are the missing pieces. We attempt to undertake this task in this paper. We present a high-level review of technologies underlying digital contact tracing, a set of metrics that are important while evaluating different contact tracing technologies, and evaluate where the different technologies stand today on this set of metrics. Our hope is two-fold: (a) Future designers of contact tracing applications can use this review paper to understand the technology landscape, and (b) Researchers can identify and solve the missing pieces of this puzzle so that we are ready to face the rest of the COVID-19 pandemic and any future pandemics. A majority of this discussion is focused on the ability to identify contact between individuals. The questions of ethics, privacy, and security of such contact tracing are briefly mentioned but not discussed in detail.

==> abstract.tex <==
\begin{abstract}
Since the start of the COVID-19 pandemic, technology enthusiasts have pushed for digital contact tracing as a critical tool for breaking the COVID-19 transmission chains. Motivated by this push, many countries and companies have created apps that enable digital contact tracing intending to identify the chain of transmission from an infected individual to others and enable early quarantine. Digital contact tracing applications like AarogyaSetu in India, TraceTogether in Singapore, SwissCovid in Switzerland, and others have been downloaded hundreds of millions of times. Yet, this technology hasn't seen the impact that we envisioned at the start of the pandemic. Some countries have rolled back their apps, while others have seen low adoption \cite{techreviewsuccess}. 

Therefore, it is prudent to ask what the technology landscape of contact-tracing looks like and what are the missing pieces. We attempt to undertake this task in this paper. We present a high-level review of technologies underlying digital contact tracing, a set of metrics that are important while evaluating different contact tracing technologies, and evaluate where the different technologies stand today on this set of metrics. Our hope is two-fold: (a) Future designers of contact tracing applications can use this review paper to understand the technology landscape, and (b) Researchers can identify and solve the missing pieces of this puzzle so that we are ready to face the rest of the COVID-19 pandemic and any future pandemics. A majority of this discussion is focused on the ability to identify contact between individuals. The questions of ethics, privacy, and security of such contact tracing are briefly mentioned but not discussed in detail.

%Cite: https://docs.google.com/spreadsheets/d/1ATalASO8KtZMx__zJREoOvFh0nmB-sAqJ1-CjVRSCOw/edit#gid=0
% Cite: https://www.technologyreview.com/2020/05/07/1000961/launching-mittr-covid-tracing-tracker/
% Cite: https://www.technologyreview.com/2020/08/10/1006174/covid-contract-tracing-app-germany-ireland-success/

\end{abstract}

==> future_direction.tex <==
\section{Path Forward}
\label{sec:future}


%\begin{itemize}
%\item Putting an infrastructure in place for contact tracing locally as well as globally for global health and wellness
%\item Privacy and county policies (EU policies are different from India)
%\item Integrating personalized health monitoring systems
%\item what should be the key elements and constraints to consider?
%\end{itemize}

In this paper, we presented various technologies that can be used for contact tracing and reviewed various pros and cons that play important role in making the design decisions of a contact tracing system. While digital contact tracing has a lot of benefits the solution should not feel and act like a surveillance system to the end-users. We also advocate the need for a global infrastructure in place as well as globally accepted privacy-preserving laws. The designed framework and system should be secure enough that agencies of the government, corporations, or any other institution should be unable to tap data resulting in the exploitation of the citizens. Finally, we strongly believe that designing an efficient privacy-preserving contact tracing system should be inter-disciplinary user-centric research and must strongly take into account the social, psychological, security, and Human-Computer Interaction aspects of users while aiding healthcare workers. 

\iffalse
Firstly, we should understand that the digital contact tracing solutions should be complementary to the manual contact tracing and not a replacement. Secondly, as discussed in earlier sections all technology based contact tracing solutions have pitfalls but that shouldn’t stop us from adopting them. Awareness of trade-offs related to each technology and paying attention to the objectives of the digital contact tracing system would help in selecting the most suitable solution. Digital contact tracing is a tool that, even with its limitations, can help reduce the disease burden on our healthcare systems by aiding the trained health professionals and volunteers. However, we must be wary of seeing technology as a savior that will magically make all problems go away. 

We strongly feel that at this point these systems require a conversation around privacy and consent while making the user in complete control of their decision without any repercussions from the government, other agencies, or corporate. Also, globally we do not have any uniformity in privacy policies for the citizens. The privacy laws in favor of citizens are very different in Europe than in Asian countries. For a globally accepted scalable solution, we also need to pay attention to privacy laws across nations.

Additionally, interpreting data collected by such apps require a lot of caution. If the apps alone decide where the focus of the healthcare system goes, it is going to be a huge injustice to a large percentage of the population who don't have digital access creating a bias in the system. If anything, more human resources should be dedicated to these areas without digital access, given that they are particularly vulnerable.

To concur, we feel that digital contact tracing has a lot of benefits with respect to ubiquity, scalability, quick reach, and precision but there are pressing issues concerning privacy and security that should not make the system feel and act like a surveillance system. While there is a need for an infrastructure to be put in place at the national level we need better privacy laws globally that are user-centric. User data leakage and use by agencies such as government that could result in the exploitation of citizens should never happen. Additionally, we need to design frameworks that are compatible with contact tracing systems that use different channels of data collection. We strongly believe that designing an efficient privacy-preserving contact tracing system should be inter-disciplinary and must give the user complete control over their data. This inter-disciplinary research should take into account the social, psychological, security, and Human-Computer Interaction aspects of users while designing solutions satisfying the needs of the healthcare workers.
\fi

==> metrics.tex <==
\section{Metrics}
\label{sec:metrics}
In the above section, we described the various technologies for designing digital contact tracing systems. But, to truly measure the desirability of a system we need to measure the efficacy and effectiveness of the solution for each of the above stated technology. In this section we identify the main metrics for measuring the effectiveness of a contact tracing system, stated as below:

\textbf{Accuracy}
The system should have both spatial and temporal accuracy to correctly identify proximity and co-location. Accuracy of users in proximity as identified the tool v/s observed ground truth is heavily tied to the location granularity of the dataset. A contact tracing system that uses Call Data Records (CDR) datasets with a coarse location granularity in the range of Kms will have very low accuracy (false positives) as compared to a Bluetooth based tool with a fine location granularity in the range of meters. Furthermore, we measure accuracy by computing the false positives and false negatives of the system. In this context, false positives identify the number of people falsely identified as being in contact, i.e. people who were never in contact with a COVID-positive patient but were identified as a contact. While false negatives identify the people who were actually in contact with a COVID-positive patient but were not identified as one. Both false positives as well as false negatives are important. On one hand, if the number of false positives is high, the contact tracing system will identify a lot more people in need of tests causing false alarm, reducing trust in the app, and overwhelming the healthcare resources. On the other hand, a high false negative value indicates that the system is missing out on identifying several colocated users thereby increasing the risk to the general population. According to a recent survey by Microsoft Research \cite{MSRStudy}, around 85\% of the surveyed population was willing to install contact tracing apps that were perfectly accurate.
%The number of false positives and false negatives is intricately linked to the accuracy of the underlying technology being used to measure the distance between individuals. If the technology can identify the difference between three feet, six feet, and nine feet, then it will perform well on this task. On the other hand, if two feet and twenty feet are interchangeable, then the technology will lead to a high number of false positives and/or false negatives.

\textbf{Privacy}
The base of contact tracing is the user health and location dataset, which makes privacy a very important metric. In fact, in the Microsoft research study quoted above \cite{MSRStudy}, privacy concerns were almost as high on people's minds as accuracy. While systems that collect absolute location information could leak details about user mobility with respect to the mobility patterns, frequency of location visits as well as details about frequent associations over time. On the other hand, systems that collect relative information could leak frequent association information as well as mobility patterns. Additionally, with a lot of social content available with people self reporting check-ins on social media, merging multiple datasets could result in a lot more privacy leakage. Understanding the system areas where privacy can be compromised and mitigating the risks of compromise is an important measure.

\textbf{Data Security and Ease of attacks}
Understanding how much data is collected per user, and mode of the data storage, Is it a single central data storage or is it a distributed data store? How easy and susceptible is the data store to attacks?

\textbf{Ubiquity}

For a contact tracing system to be effective, a large percentage of the population must adopt it. Accordingly to \cite{WSJ-TT} about 80\% of the user population needs to use the contracting app for it to be effective. Additionally, this problem arises not only because of the need for users to download, install the app and consent the collection of data as in the case of Bluetooth based apps but also to keep the app running and enabled all the time. Most Bluetooth enabled apps drain energy very quickly resulting in users disabling the apps. This on a bigger scale results in an inefficient and incorrect contact tracing system. From the user adoption perspective, systems that use an existing data source collected passively for alternate reasons such as WiFi logs based system that uses network logs collected for network analysis, do not suffer from this problem. Once a user gives consent to data collection the network-centric system does not need any apps to run on individual mobile devices.

Large scale user adoption has 2 main aspects:
\begin{itemize}
\item Universal availability: The technology used for proximity detection has to be universal: it must be compatible with smartphones using outdated software. To understand why this is important, consider the chart of Android users below. Even if one restricts the app to Android 8.0 that was launched in mid-2017, about 25 percent of global smartphone users won't be able to use it. Therefore, any apps that use capabilities available only in modern mobile operating systems won't scale.
\item Scalable design: The app must be able to identify contact not only in homes where few smartphones talk to each other and identify their distance, but also in crowded retail stores, subways, and supermarkets, that have hundreds of people walking around. The design of the apps must be able to handle such large traffic and measure accurate proximity within this large group of people. The other aspect of the scalable design is the ability to not crash when tens of millions of people end up using the app -- this is the scale that most internet applications dream of. For example, AarogyaSetu, the official Indian government application for digital contact tracing crossed 100 million downloads. Apps operating at such a scale need to follow skillful engineering practices.
\end{itemize}

\iffalse
This section describes the metrics to measure efficacy and effectiveness of digital contact tracing solutions for each of the above stated technology.
\begin{itemize}
\item Spatial and Temporal Accuracy
\item Privacy
\item Data Security and ease of attacks
\item Percentage population adoption needed for the technology to be successful 
\end{itemize}

Metrics of Interest

Given the importance of digital contact tracing, you will soon hear (or are hearing) about lots of different solutions to enable contact tracing using smartphones. If you are a policymaker, or a retail store manager, or a city administrator, or just someone concerned about COVID-19, what questions should you ask about the contact tracing apps that the technologists are selling to you?
Accuracy

Accuracy is, of course, one of the most important parameters, i.e. any solution that we use should be able to correctly identify contact. Generally, a contact is defined as being closer than 6 feet for more than 10 minutes. According to a recent survey by Microsoft Research, around 85\% of the surveyed population was willing to install contact tracing apps that were perfectly accurate. In terms of measuring accuracy, there are two kinds of errors that we care about:

    False positives: The number of people falsely identified as being in contact, i.e. people who were never in contact with a COVID-positive patient, but were identified as a contact.
    False negatives: The number of people falsely identified as not being in contact, i.e. people who were actually in contact with a COVID-positive patient, but were not identified as one.

No alt text provided for this image

As you can imagine, both false positives and false negatives are important numbers. If the number of false positives is high, the app will recommend a lot more tests than needed, thereby causing false alarms, reducing trust in the app, and overwhelming the healthcare resources. On the other hand, if the number of false negatives is high, it will miss out on high-risk individuals and increase the risk to the general population.

The number of false positives and false negatives is intricately linked to the accuracy of the underlying technology being used to measure the distance between individuals. If the technology can identify the difference between three feet, six feet, and nine feet, then it will perform well on this task. On the other hand, if two feet and twenty feet are interchangeable, then the technology will lead to a high number of false positives and/or false negatives.
Privacy

When it comes to apps that track our proximity to others and have access to our health information, privacy is a very important metric. In fact, in the Microsoft research study I quoted above, privacy concerns were almost as high on people's minds as accuracy. The graph below is a summary of their results.
No alt text provided for this image

Source: How good is good enough for COVID19 apps? The influence of benefits, accuracy, and privacy on willingness to adopt. Kaptchuk et al. https://arxiv.org/pdf/2005.04343.pdf

There are varying levels of information that these apps can leak about you:

    Personal Information: Your name, address, health history, COVID-19 status
    Location: Your fine-grained location data, what places you visit, when you go, who do you go there with?
    Associations: Who do you travel with, what people do you meet, how frequently do you meet them?

Not all apps collect all of this information. The least privacy-invasive apps will just collect association data and not expose it to anyone but you. The most privacy-invasive apps will collect all of this data and access this data externally. Before you adopt an app or endorse it, be sure to look out for the data it collects and remember to check who can access that data.
Ubiquity

Public health officials believe that any contact tracing app needs to be used by 60 percent of the population for it to be effective. Achieving this density of adoption imposes two requirements:

Universal availability: The technology used for proximity detection has to be universal: it must be compatible with smartphones using outdated software. To understand why this is important, consider the chart of Android users below. Even if one restricts the app to Android 8.0 that was launched in mid-2017, about 25% of global smartphone users won't be able to use it. Therefore, any apps that use capabilities available only in modern mobile operating systems won't scale.
No alt text provided for this image

Source: Android Version Market Share worldwide https://gs.statcounter.com/android-version-market-share/mobile-tablet/worldwide

Scalable design: The app must be able to identify contact not only in homes where few smartphones talk to each other and identify their distance, but also in crowded retail stores, subways, and supermarkets, that have hundreds of people walking around. The design of the apps must be able to handle such large traffic and measure accurate proximity within this large group of people. The other aspect of scalable design is the ability to not crash when tens of millions of people end up using the app -- this is the scale that most internet applications dream of. For example, AarogyaSetu, the official Indian government application for digital contact tracing recently crossed 100 million downloads. Apps operating at such a scale need to follow skillful engineering practices.

In summary, if you are a decision-maker that needs to choose an app for yourself, your business, county, city, or country, here is a list of questions to ask:

    How accurate is the technology? What is the percentage of false positives and false negatives?
    What data does it collect? What data can be accessed on the cloud? Who has access to this data?
    What is the minimum requirement for a device that can install and run this app?
    How many people can it track in a single location?
    How many simultaneous users can it handle?
    
\fi

==> ref.tex <==
% This file serves as a scratch pad for adding quick references to read. 

%Currently, this is just a dummy file to hold list of all papers referenced. A paper.bib file will be created.

==> system_design.tex <==
\section{System Design Considerations} 
\label{sec:system_design}


\begin{itemize}
\item  what are the challenge areas in system design, implementation, and deployment with respect to contact tracing?
\item what are the other challenge areas with respect to policy, human-wellness, etc that should be considered?
\end{itemize}
